WiCkeD: A Simple Method to Make Multiple Choice Benchmarks More Challenging

We introduce WiCkeD, a simple method to increase the complexity of existing multiple-choice benchmarks by randomly replacing a choice with "None of the above", a method often used in educational tests. We show that WiCkeD can be automatically applied to any existing benchmark, making it more challenging. We apply WiCkeD to 6 popular benchmarks and use it to evaluate 18 open-weight LLMs. The performance of the models drops 12.1 points on average with respect to the original versions of the datasets. When using chain-of-thought on 3 MMLU datasets, the performance drop for the WiCkeD variant is similar to the one observed when using the LLMs directly, showing that WiCkeD is also challenging for models with enhanced reasoning abilities. WiCkeD also uncovers that some models are more sensitive to the extra reasoning required, providing additional information with respect to the original benchmarks. We relase our code and data at https://github.com/ahmedselhady/wicked-benchmarks.

==> latex/figures/arc_challenge_detailed.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1.\linewidth,]{latex/imgs/detailed/arc_challenge.wickd_org_acc.hf_models.pdf}
\caption{Detailed Performances on the original and \wicds Arc Challenge benchmark }
\label{fig:arc-detailed}
\end{figure*} 




==> latex/figures/arc_examples.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1\columnwidth]{latex/imgs/allenai_arc.png}
\caption{Examples from the AllenAi Arc challenge using \wicd. We show 3-shot for brevity, but 5-shot was actually used in the experiments for the main results. The first few-shot example does not include \nota~ option because it was classified as SBA question.}
\label{fig:arc-examples}
\end{figure} 

==> latex/figures/csqa_examples.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1\columnwidth]{latex/imgs/csqa.png}
\caption{Examples from the Common-sense QA using \wicd.  We show 3-shot for brevity, but 5-shot was actually used in the experiments for the main results. The first few-shot example does not include \nota~ option because it was classified as SBA question. }
\label{fig:csqa-examples}
\end{figure} 

==> latex/figures/degradation.cot.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1.\columnwidth]{latex/imgs/mean.cot-and-mcq.pdf}
\caption{Models' performances on the original and \wicds MMLU, MMLU-pro, and MMLU-Redux benchmarks with multiple-choice prompting and chain-of-thoughts.}
\label{fig:cot-res}
\end{figure} 

==> latex/figures/degradation.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1.\columnwidth]{latex/imgs/mean.wickd_org_acc.hf_models.pdf}
\caption{Models' performances on the \wicd\space variant and the original benchmarks. Qwen2.5-72B and Llama3.1-70B models are the best performing on both variants. However, Qwen2.5-7B and Qwen2.514B models experience the largest degradation, raising concerns about whether their performances were overestimated.}
\label{fig:main-res}
\end{figure} 


==> latex/figures/instrut_vs_base.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1.\columnwidth]{latex/imgs/piechart.png}
\caption{The changes in models' answers of the original benchmarks and the \wicds variant using chain-of-thoughts. }
\label{fig:piechart}
\end{figure} 

==> latex/figures/mmlu_cs_examples.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1\columnwidth]{latex/imgs/mmlu_computer_science.png}
\caption{Examples from the MMLU computer science task using \wicd.  We show 3-shot for brevity, but 5-shot was actually used in the experiments for the main results.}
\label{fig:mmlu-cs-examples}
\end{figure} 

==> latex/figures/mmlu_detailed_1.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_1.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (1/7)}
\label{fig:mmlu-det-1}
\end{figure*} 




==> latex/figures/mmlu_detailed_2.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_2.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (2/7)}
\label{fig:mmlu-det-2}
\end{figure*} 




==> latex/figures/mmlu_detailed_3.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_3.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (3/7)}
\label{fig:mmlu-det-3}
\end{figure*} 




==> latex/figures/mmlu_detailed_4.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_4.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (4/7)}
\label{fig:mmlu-det-4}
\end{figure*} 




==> latex/figures/mmlu_detailed_5.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_5.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (5/7)}
\label{fig:mmlu-det-5}
\end{figure*} 




==> latex/figures/mmlu_detailed_6.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_6.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (6/7)}
\label{fig:mmlu-det-6}
\end{figure*} 




==> latex/figures/mmlu_detailed_7.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth]{latex/imgs/detailed/mmlu_7.png}
\caption{Detailed Performances on the original and \wicds MMLU sub tasks (7/7)}
\label{fig:mmlu-det-7}
\end{figure*} 




==> latex/figures/mmlu_pro_detailed_1.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1.\linewidth,  height=0.8\textheight]{latex/imgs/detailed/mmlu_pro_1.png}
\caption{Detailed Performances on the original and \wicds MMLU-Pro sub tasks (1/2) }
\label{fig:mmlu-pro-detailed}
\end{figure*} 




==> latex/figures/mmlu_pro_detailed_2.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1.\linewidth,  height=0.7\textheight]{latex/imgs/detailed/mmlu_pro_2.png}
\caption{Detailed Performances on the original and \wicds MMLU-Pro sub tasks (2/2) }
\label{fig:mmlu-pro-detailed2}
\end{figure*} 




==> latex/figures/mmlu_redux_detailed_1.tex <==
\begin{figure*}[th!]
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_redux_1.png}
\caption{Detailed Performances on the original and \wicds MMLU-Redux sub tasks (1/3)}
\label{fig:redux-det-1}
\end{figure*} 




==> latex/figures/mmlu_redux_detailed_2.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_redux_2.png}
\caption{Detailed Performances on the original and \wicds MMLU-Redux sub tasks (2/3)}
\label{fig:redux-det-2}
\end{figure*} 




==> latex/figures/mmlu_redux_detailed_3.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=1\linewidth,  height=\textheight]{latex/imgs/detailed/mmlu_redux_3.png}
\caption{Detailed Performances on the original and \wicds MMLU-Redux sub tasks (3/3)}
\label{fig:redux-det-3}
\end{figure*} 




==> latex/figures/mmlu_redux_examples.tex <==
\begin{figure}[th!]
\centering
\includegraphics[width=1\columnwidth]{latex/imgs/mmlu_redux.png}
\caption{Examples from the MMLU-Redux using \wicd. We show 3-shot for brevity, but 5-shot was actually used in the experiments for the main results. }
\label{fig:mmlur-examples}
\end{figure} 

==> latex/figures/sba_vs_sca.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1.\columnwidth]{latex/imgs/sba_example.drawio.png}
\caption{Applying \wicds on a single best answer (SBA) example (best answer D, second best answer A) would lead to an incoherent \wicds variant (incorrectly having \nota ~as the gold correct answer instead of A). We thus copy SBA examples verbatim, see \S~\ref{sec:coherence} for details.  }
%\caption{A single best answer (SBA) example (best answer D, second best answer A), which would lead to an incoherent \wicds variant, with \nota ~as the gold correct answer instead of A. We thus copy SBA examples verbatim, see \S~\ref{sec:coherence} for details.  }
\label{fig:sba-vs-sca}
\end{figure} 

==> latex/figures/wicked.tex <==
\begin{figure*}[th!]
\centering
\includegraphics[width=0.7\linewidth]{latex/imgs/wildcard.drawio.png}
\caption{Two samples from MMLU-Pro (left) and its \wicds variant (right), where \textit{Hydrogen} and \textit{Centrifugal} were removed. Correct answers in bold. Llama-3.1 8B correctly answers both original questions but fails on the \wicds variant for the second question. The probability distribution of the model for each answer is also shown.}
\label{fig:wicked}
\end{figure*} 




==> latex/tables/SbaVsSCA.tex <==

\begin{table}[t!]
% \resizebox{width=1\columnwidth}{!}{
\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{l|l|}
\toprule
\multirow{2}{*}{\rotatebox[origin=c]{90}{Single Correct Answer}}&\makecell[l]{\textbf{Question:} The limbic system plays an important role in \\ A) maintaining balance. \\ \textcolor{red}{B) regulating emotion.} \\ C) monitoring arousal. \\ D) ...}\\
% \bottomrule
&\cellcolor{blue!25} \makecell[l]{\textbf{Question:} The limbic system plays an important role in \\ A) maintaining balance. \\ \textcolor{red}{B) regulating emotion.} \\ C) monitoring arousal. \\ D) None of the above}\\
\toprule
\multirow{2}{*}{\rotatebox[origin=c]{90}{Single Best Answer}}&\makecell[l]{\textbf{Question:} Which definition best describes media convergence? \\ A) The conglomeration of media outlets into large corporations. \\ B) The many differing views and cultures expressed in modern media. \\ C)Information being delivered in different formats via various digital channels. \\ \textcolor{red}{D) merging of different forms of media into a unified digital format}}\\
& \cellcolor{blue!25} \makecell[l]{\textbf{Question:} Which definition best describes media convergence? \\ \textcolor{red}{A) The conglomeration of media outlets into large corporations.} \\ B) The many differing views and cultures expressed in modern media. \\ C)Information being delivered in different formats via various digital channels. \\ D) None of the above}\\
\end{tabular}
\end{adjustbox}
% }
\caption{\todo{add caption}}
\label{tab:sba-vs-sca}
\end{table}


==> latex/tables/gpt_annotation_prompt.tex <==
\begin{table*}[th!]
\centering
\begin{adjustbox}{max width=1.\linewidth}
\begin{tabular}{|l|}
\toprule
% \textbf{Column 1} & \textbf{Column 2} \\ \hline
\texttt{"A single correct answer question is a question that can have exactly one correct answer from a given set of choices.}\\
\texttt{A single best answer question can have a most appropriate answer (for example, if this answer is omitted, another answer will be correct). 
}\\
\texttt{Classify the following questions into SBA and non-SBA questions. Assign a label of 1 if the question is a SBA question and a label of 0 otherwise.
} \\
\texttt{Question: \{question\}
Class:" 
} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{SBA Annotation Prompt Template}
\label{tab:prompt_template}
\end{table*}



==> latex/tables/mean.wickd_org_acc.hf_models.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{0.9} 
\begin{adjustbox}{max width=1.\columnwidth}

\begin{tabular}{lrcrrr}
\toprule
\textbf{Model} & \textbf{Size} & \makecell{\textbf{IT}} & \textbf{Original}  & \textbf{\wicd} &  \multicolumn{1}{c}{$\mathbf{\Delta}$} \\
\midrule
DS-R1-Llama & 8B & - & 56.6 & 48.6 &-7.9  {\scriptsize $\pm 1.1\%$}\\
DS-R1-Qwen& 7B & -  & 60.8 & 53.4  &-7.3 {\scriptsize $\pm 1.6\%$}\\
\midrule
\multirow{4}{*}{Llama-3.1} & 8B & - & 61.4 & 52.2  &-9.2 {\scriptsize $\pm 1.7\%$}  \\
& 8B & $\checkmark$ & 66.0 & 55.0 &-11.0  {\scriptsize $\pm 0.9\%$}\\
& 70B & - & 76.8 & 67.0  &-9.8 {\scriptsize $\pm 2.1\%$}\\
& 70B & $\checkmark$ & 77.1 & 64.5  & -12.6 {\scriptsize $\pm 1.3\%$}\\
\midrule
\multirow{2}{*}{Mistral} & 7B & - & 59.8 & 46.5 &-13.2 {\scriptsize $\pm 1.2\%$} \\
& 7B & $\checkmark $& 59.0  & 47.2  &-11.8 {\scriptsize $\pm 1.1\%$}\\
\midrule
\multirow{6}{*}{Qwen-2.5}& 7B & - & 74.7 & 54.9 &-19.7 {\scriptsize $\pm 1.5\%$}\\
& 7B & $\checkmark $& 73.5 & 59.0 &-14.5  {\scriptsize $\pm 1.3\%$}\\
& 14B & - & 78.9 & 66.3  &-12.6 {\scriptsize $\pm 2.1\%$}\\
& 14B & $\checkmark $& 78.9 & 66.6  &-12.3  {\scriptsize $\pm 1.8\%$}\\
& 72B & - & 84.6 & 72.6 &-12.0 {\scriptsize $\pm 0.9\%$}\\
& 72B &  $\checkmark $ & 82.6 & 69.3 & -13.3 {\scriptsize $\pm 1.0\%$}\\
\midrule
\multirow{4}{*}{Gemma-2}& 9B & - & 67.3 & 56.3 &-10.9 {\scriptsize $\pm 1.2\%$}\\
& 9B & $\checkmark $& 73.3 & 57.6  &-15.7  {\scriptsize $\pm 1.2\%$}\\
& 27B & - & 68.0  & 54.6  &-13.4 {\scriptsize $\pm 2.0\%$}\\
& 27B & $\checkmark $ & 74.8 & 61.9 &-12.9 {\scriptsize $\pm 2.3\%$}\\
\bottomrule
\textbf{Average} &&& \textbf{70.78} & \textbf{58.52} &\cellcolor{red!25} \textbf{-12.2} {\scriptsize $\pm 26.3\%$}\\ 
\toprule
\end{tabular}
\end{adjustbox}
\caption{Average performance on original and \wicds variants of the six benchmarks. IT: instruction-tuned. $\mathbf{\Delta}$: degradation from original performance}
%Models' performances on the \wicd\space variant and the original benchmarks. Qwen2.5-72B and Llama3.1-70B models are the best performing on both variants. However, Qwen2.5-7B and Qwen2.514B models experience the largest degradation, raising concerns about whether their performances were overestimated. $\mathbf{\Delta}$ : mean and standard deviation of degradation from original performance}
\label{tab:detailed-results}

\end{table}

==> latex/tables/mean.wickd_org_cot.hf_models.tex <==


\begin{table}[t!]
\renewcommand{\arraystretch}{0.9} 
\begin{adjustbox}{max width=1.\columnwidth}

\begin{tabular}{lrccrrcr}
\toprule
&&&\multicolumn{2}{c}{\textbf{Direct}}&&\multicolumn{2}{c}{\textbf{CoT}}\\
\cmidrule{4-5} \cmidrule{7-8}
\textbf{Model} & \textbf{Size} & \makecell{\textbf{IT}} 
&\textbf{\wicd} 
& $\mathbf{\Delta}$
&&\textbf{\wicd}&$\mathbf{\Delta}$\\
\midrule
DS-R1-Llama & 8B & - &  30.3 & -4.1&&80.1 & -2.0 \\
DS-R1-Qwen& 7B & -  &  30.6 & -4.3&&74.9  &-2.5 \\
\midrule
\multirow{2}{*}{Llama-3.1} & 8B & - & 39.7 &-3.2&& 53.9  &-5.8  \\
& 8B & $\checkmark$ & 43.6 &-2.7&& 57.2 &-3.4  \\
\midrule
\multirow{2}{*}{Mistral} & 7B & -  &35.9 &-3.4&& 36.3&-11.62  \\
& 7B & $\checkmark $ & 33.5 &-5.7&& 43.8 &-4.97 \\
\midrule
\multirow{4}{*}{Qwen-2.5}& 7B & -  & 45.5 &-6.9&& 43.0 &-14.62 \\
& 7B & $\checkmark $ & 47.1 &-5.3&& 55.4 &-1.73  \\
& 14B & - & 55.6 &-3.6&& 61.5 &-3.97 \\
& 14B & $\checkmark $&  56.7 &-3.4&& 64.0 &-1.43  \\
\midrule
\multirow{4}{*}{Gemma-2}& 9B & -  & 36.1 &-12.2&& 41.2 &-8.93 \\
& 9B & $\checkmark $& 44.1 &-9.3&& 56.3 &-4.36  \\
& 27B & -  & 36.1&-10.8&& 59.2 &-4.07\\
& 27B & $\checkmark $  & 51.3 &-3.8&& 60.3 &-3.77 \\
\bottomrule
\textbf{Average} &&&\textbf{41.86} &\cellcolor{red!25} \textbf{-5.62} && \textbf{\textbf{56.26}} &\cellcolor{red!25} \textbf{-5.24}\\ 
\toprule
\end{tabular}

\end{adjustbox}
\caption{Performance on \wicds variants for MMLU, MMLU-pro, and MMLU-Redux without and with CoT.  IT: instruction-tuned. $\mathbf{\Delta}$: degradation from the original benchmark.}
\label{tab:detailed-results-cot}

\end{table}


==> latex/tables/mmlu_original_detailed.tex <==
\begin{sidewaystable}

\begin{tabular}{lrlrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
    \toprule
    model & size & type & mmlu & humanities & formal logic & high school european history & high school us history & high school world history & international law & jurisprudence & logical fallacies & moral disputes & moral scenarios & philosophy & prehistory & professional law & world religions & other & business ethics & clinical knowledge & college medicine & global facts & human aging & management & marketing & medical genetics & miscellaneous & nutrition & professional accounting & professional medicine & virology & social sciences & econometrics & high school geography & high school government and politics & high school macroeconomics & high school microeconomics & high school psychology & human sexuality & professional psychology & public relations & security studies & sociology & us foreign policy & stem & abstract algebra & anatomy & astronomy & college biology & college chemistry & college computer science & college mathematics & college physics & computer security & conceptual physics & electrical engineering & elementary mathematics & high school biology & high school chemistry & high school computer science & high school mathematics & high school physics & high school statistics & machine learning \\
    \midrule
    DeepSeek-R1-Distill-Llama & 8B & original & 0.556 & 0.506 & 0.460 & 0.715 & 0.676 & 0.776 & 0.661 & 0.630 & 0.632 & 0.598 & 0.321 & 0.640 & 0.614 & 0.404 & 0.713 & 0.618 & 0.600 & 0.611 & 0.607 & 0.310 & 0.592 & 0.757 & 0.821 & 0.630 & 0.702 & 0.670 & 0.408 & 0.555 & 0.458 & 0.651 & 0.368 & 0.732 & 0.741 & 0.505 & 0.559 & 0.760 & 0.702 & 0.562 & 0.673 & 0.735 & 0.781 & 0.820 & 0.475 & 0.370 & 0.511 & 0.553 & 0.632 & 0.340 & 0.540 & 0.410 & 0.314 & 0.640 & 0.455 & 0.441 & 0.479 & 0.674 & 0.448 & 0.580 & 0.352 & 0.344 & 0.449 & 0.348 \\
    DeepSeek-R1-Distill-Llama & 8B & wickd & 0.487 & 0.471 & 0.468 & 0.630 & 0.681 & 0.743 & 0.595 & 0.611 & 0.528 & 0.520 & 0.325 & 0.531 & 0.574 & 0.388 & 0.556 & 0.529 & 0.490 & 0.581 & 0.503 & 0.190 & 0.529 & 0.544 & 0.662 & 0.610 & 0.596 & 0.565 & 0.340 & 0.526 & 0.398 & 0.554 & 0.325 & 0.581 & 0.653 & 0.490 & 0.487 & 0.683 & 0.580 & 0.487 & 0.527 & 0.482 & 0.682 & 0.610 & 0.403 & 0.190 & 0.452 & 0.500 & 0.535 & 0.210 & 0.420 & 0.280 & 0.343 & 0.620 & 0.374 & 0.331 & 0.431 & 0.558 & 0.429 & 0.590 & 0.296 & 0.291 & 0.343 & 0.312 \\
    DeepSeek-R1-Distill-Qwen & 1.5B & original & 0.374 & 0.320 & 0.333 & 0.352 & 0.319 & 0.397 & 0.479 & 0.417 & 0.374 & 0.364 & 0.259 & 0.421 & 0.386 & 0.269 & 0.322 & 0.402 & 0.430 & 0.404 & 0.329 & 0.330 & 0.399 & 0.369 & 0.641 & 0.470 & 0.433 & 0.376 & 0.273 & 0.335 & 0.386 & 0.415 & 0.351 & 0.485 & 0.383 & 0.418 & 0.525 & 0.428 & 0.412 & 0.327 & 0.418 & 0.408 & 0.468 & 0.510 & 0.388 & 0.390 & 0.326 & 0.342 & 0.285 & 0.350 & 0.340 & 0.360 & 0.245 & 0.400 & 0.421 & 0.483 & 0.418 & 0.410 & 0.429 & 0.460 & 0.341 & 0.245 & 0.528 & 0.411 \\
    DeepSeek-R1-Distill-Qwen & 1.5B & wickd & 0.310 & 0.292 & 0.317 & 0.339 & 0.309 & 0.367 & 0.364 & 0.398 & 0.307 & 0.361 & 0.263 & 0.309 & 0.287 & 0.259 & 0.269 & 0.312 & 0.250 & 0.298 & 0.283 & 0.290 & 0.336 & 0.311 & 0.376 & 0.400 & 0.347 & 0.255 & 0.291 & 0.272 & 0.271 & 0.333 & 0.351 & 0.318 & 0.368 & 0.321 & 0.366 & 0.352 & 0.321 & 0.299 & 0.336 & 0.298 & 0.333 & 0.460 & 0.310 & 0.330 & 0.267 & 0.296 & 0.278 & 0.250 & 0.250 & 0.280 & 0.255 & 0.290 & 0.353 & 0.310 & 0.333 & 0.352 & 0.305 & 0.350 & 0.304 & 0.252 & 0.338 & 0.330 \\
    DeepSeek-R1-Distill-Qwen & 7B & original & 0.541 & 0.447 & 0.516 & 0.600 & 0.598 & 0.700 & 0.620 & 0.611 & 0.656 & 0.538 & 0.258 & 0.585 & 0.519 & 0.357 & 0.526 & 0.547 & 0.570 & 0.536 & 0.486 & 0.290 & 0.561 & 0.718 & 0.761 & 0.520 & 0.631 & 0.536 & 0.401 & 0.412 & 0.452 & 0.635 & 0.570 & 0.667 & 0.668 & 0.603 & 0.756 & 0.723 & 0.534 & 0.533 & 0.555 & 0.669 & 0.627 & 0.710 & 0.584 & 0.460 & 0.407 & 0.625 & 0.590 & 0.480 & 0.570 & 0.470 & 0.451 & 0.690 & 0.685 & 0.614 & 0.651 & 0.655 & 0.567 & 0.700 & 0.467 & 0.570 & 0.681 & 0.438 \\
    DeepSeek-R1-Distill-Qwen & 7B & wickd & 0.485 & 0.422 & 0.500 & 0.539 & 0.554 & 0.629 & 0.554 & 0.611 & 0.583 & 0.497 & 0.291 & 0.502 & 0.466 & 0.344 & 0.439 & 0.489 & 0.540 & 0.494 & 0.428 & 0.270 & 0.507 & 0.534 & 0.662 & 0.500 & 0.562 & 0.480 & 0.344 & 0.404 & 0.404 & 0.558 & 0.518 & 0.591 & 0.601 & 0.531 & 0.706 & 0.670 & 0.458 & 0.480 & 0.482 & 0.392 & 0.612 & 0.580 & 0.504 & 0.280 & 0.385 & 0.539 & 0.521 & 0.430 & 0.510 & 0.460 & 0.373 & 0.650 & 0.515 & 0.490 & 0.598 & 0.590 & 0.507 & 0.630 & 0.400 & 0.470 & 0.551 & 0.402 \\
    Llama-3.1 & 8B & original & 0.647 & 0.593 & 0.468 & 0.770 & 0.819 & 0.827 & 0.843 & 0.722 & 0.785 & 0.708 & 0.384 & 0.746 & 0.713 & 0.482 & 0.819 & 0.719 & 0.670 & 0.725 & 0.659 & 0.330 & 0.713 & 0.835 & 0.863 & 0.800 & 0.811 & 0.797 & 0.493 & 0.699 & 0.560 & 0.760 & 0.474 & 0.838 & 0.881 & 0.621 & 0.739 & 0.853 & 0.824 & 0.711 & 0.691 & 0.727 & 0.891 & 0.890 & 0.548 & 0.360 & 0.600 & 0.717 & 0.778 & 0.450 & 0.450 & 0.320 & 0.471 & 0.810 & 0.587 & 0.641 & 0.415 & 0.784 & 0.557 & 0.680 & 0.396 & 0.391 & 0.532 & 0.411 \\
    Llama-3.1 & 8B & wickd & 0.568 & 0.526 & 0.508 & 0.709 & 0.809 & 0.785 & 0.636 & 0.667 & 0.607 & 0.595 & 0.311 & 0.637 & 0.608 & 0.462 & 0.620 & 0.614 & 0.600 & 0.558 & 0.549 & 0.280 & 0.596 & 0.709 & 0.658 & 0.630 & 0.677 & 0.699 & 0.496 & 0.695 & 0.482 & 0.664 & 0.439 & 0.707 & 0.762 & 0.531 & 0.647 & 0.776 & 0.702 & 0.606 & 0.582 & 0.690 & 0.766 & 0.720 & 0.492 & 0.350 & 0.541 & 0.625 & 0.688 & 0.440 & 0.450 & 0.380 & 0.431 & 0.660 & 0.460 & 0.621 & 0.389 & 0.697 & 0.493 & 0.580 & 0.311 & 0.377 & 0.505 & 0.375 \\
    
    
    Llama-3.1 & 70B & original & 0.780 & 0.744 & 0.659 & 0.867 & 0.951 & 0.937 & 0.884 & 0.870 & 0.890 & 0.853 & 0.616 & 0.865 & 0.895 & 0.619 & 0.918 & 0.821 & 0.810 & 0.830 & 0.780 & 0.460 & 0.825 & 0.893 & 0.923 & 0.860 & 0.905 & 0.876 & 0.621 & 0.886 & 0.584 & 0.874 & 0.649 & 0.934 & 0.974 & 0.815 & 0.878 & 0.936 & 0.870 & 0.845 & 0.755 & 0.853 & 0.935 & 0.940 & 0.702 & 0.420 & 0.770 & 0.914 & 0.931 & 0.550 & 0.680 & 0.550 & 0.500 & 0.870 & 0.826 & 0.738 & 0.606 & 0.897 & 0.729 & 0.860 & 0.478 & 0.517 & 0.718 & 0.661 \\
    Llama-3.1 & 70B & wickd & 0.702 & 0.670 & 0.619 & 0.812 & 0.936 & 0.895 & 0.744 & 0.787 & 0.724 & 0.705 & 0.565 & 0.756 & 0.802 & 0.571 & 0.708 & 0.737 & 0.720 & 0.736 & 0.647 & 0.470 & 0.744 & 0.748 & 0.722 & 0.840 & 0.828 & 0.742 & 0.617 & 0.879 & 0.476 & 0.794 & 0.596 & 0.803 & 0.917 & 0.710 & 0.798 & 0.895 & 0.779 & 0.763 & 0.600 & 0.776 & 0.871 & 0.830 & 0.626 & 0.520 & 0.637 & 0.776 & 0.847 & 0.590 & 0.590 & 0.500 & 0.588 & 0.710 & 0.685 & 0.628 & 0.508 & 0.790 & 0.650 & 0.790 & 0.393 & 0.497 & 0.681 & 0.616 \\
    Llama-3.1-Instruct & 8B & original & 0.677 & 0.634 & 0.548 & 0.758 & 0.819 & 0.857 & 0.835 & 0.796 & 0.822 & 0.734 & 0.537 & 0.717 & 0.719 & 0.500 & 0.819 & 0.733 & 0.710 & 0.732 & 0.665 & 0.410 & 0.695 & 0.845 & 0.868 & 0.850 & 0.830 & 0.784 & 0.504 & 0.761 & 0.530 & 0.774 & 0.535 & 0.833 & 0.891 & 0.672 & 0.773 & 0.870 & 0.786 & 0.712 & 0.718 & 0.739 & 0.876 & 0.890 & 0.591 & 0.350 & 0.674 & 0.757 & 0.799 & 0.470 & 0.550 & 0.430 & 0.402 & 0.800 & 0.600 & 0.669 & 0.466 & 0.826 & 0.611 & 0.780 & 0.422 & 0.490 & 0.551 & 0.562 \\
    Llama-3.1-Instruct & 8B & wickd & 0.602 & 0.579 & 0.619 & 0.727 & 0.819 & 0.797 & 0.636 & 0.694 & 0.669 & 0.616 & 0.518 & 0.630 & 0.636 & 0.471 & 0.626 & 0.639 & 0.650 & 0.608 & 0.572 & 0.380 & 0.574 & 0.718 & 0.688 & 0.720 & 0.733 & 0.637 & 0.500 & 0.739 & 0.464 & 0.683 & 0.430 & 0.753 & 0.751 & 0.579 & 0.672 & 0.806 & 0.687 & 0.634 & 0.536 & 0.698 & 0.756 & 0.730 & 0.520 & 0.320 & 0.578 & 0.645 & 0.729 & 0.460 & 0.430 & 0.360 & 0.382 & 0.640 & 0.494 & 0.607 & 0.418 & 0.723 & 0.562 & 0.640 & 0.378 & 0.411 & 0.509 & 0.536 \\
    Mistral-Instruct & 7B & original & 0.587 & 0.527 & 0.421 & 0.739 & 0.775 & 0.755 & 0.793 & 0.741 & 0.748 & 0.673 & 0.320 & 0.675 & 0.657 & 0.379 & 0.842 & 0.660 & 0.590 & 0.672 & 0.578 & 0.340 & 0.632 & 0.767 & 0.863 & 0.650 & 0.765 & 0.686 & 0.465 & 0.629 & 0.488 & 0.694 & 0.412 & 0.768 & 0.819 & 0.572 & 0.622 & 0.787 & 0.718 & 0.624 & 0.682 & 0.710 & 0.846 & 0.820 & 0.502 & 0.310 & 0.622 & 0.618 & 0.701 & 0.390 & 0.530 & 0.340 & 0.373 & 0.720 & 0.523 & 0.600 & 0.370 & 0.732 & 0.483 & 0.630 & 0.330 & 0.358 & 0.477 & 0.464 \\
    Mistral-Instruct & 7B & wickd & 0.519 & 0.479 & 0.405 & 0.691 & 0.745 & 0.717 & 0.645 & 0.630 & 0.571 & 0.566 & 0.358 & 0.543 & 0.577 & 0.357 & 0.637 & 0.578 & 0.560 & 0.570 & 0.514 & 0.360 & 0.578 & 0.670 & 0.684 & 0.570 & 0.654 & 0.565 & 0.447 & 0.603 & 0.440 & 0.600 & 0.351 & 0.621 & 0.679 & 0.472 & 0.542 & 0.730 & 0.603 & 0.533 & 0.564 & 0.637 & 0.731 & 0.720 & 0.443 & 0.410 & 0.526 & 0.553 & 0.569 & 0.480 & 0.330 & 0.330 & 0.353 & 0.570 & 0.404 & 0.455 & 0.331 & 0.626 & 0.409 & 0.570 & 0.319 & 0.351 & 0.477 & 0.438 \\
    Mistral & 7B & original & 0.615 & 0.563 & 0.373 & 0.758 & 0.809 & 0.747 & 0.810 & 0.759 & 0.804 & 0.673 & 0.351 & 0.704 & 0.660 & 0.454 & 0.848 & 0.687 & 0.590 & 0.657 & 0.636 & 0.350 & 0.686 & 0.757 & 0.859 & 0.710 & 0.796 & 0.729 & 0.507 & 0.651 & 0.518 & 0.713 & 0.456 & 0.763 & 0.865 & 0.592 & 0.630 & 0.800 & 0.771 & 0.663 & 0.655 & 0.706 & 0.846 & 0.860 & 0.528 & 0.310 & 0.600 & 0.678 & 0.688 & 0.530 & 0.490 & 0.400 & 0.402 & 0.760 & 0.562 & 0.559 & 0.394 & 0.745 & 0.532 & 0.690 & 0.363 & 0.377 & 0.509 & 0.518 \\
    Mistral & 7B & wickd & 0.544 & 0.508 & 0.389 & 0.715 & 0.779 & 0.734 & 0.628 & 0.685 & 0.577 & 0.604 & 0.334 & 0.572 & 0.593 & 0.428 & 0.661 & 0.598 & 0.550 & 0.566 & 0.526 & 0.270 & 0.605 & 0.660 & 0.662 & 0.660 & 0.691 & 0.611 & 0.454 & 0.647 & 0.482 & 0.626 & 0.325 & 0.657 & 0.762 & 0.531 & 0.542 & 0.745 & 0.641 & 0.570 & 0.527 & 0.641 & 0.731 & 0.750 & 0.464 & 0.340 & 0.474 & 0.612 & 0.590 & 0.500 & 0.370 & 0.360 & 0.314 & 0.610 & 0.447 & 0.476 & 0.354 & 0.674 & 0.473 & 0.610 & 0.348 & 0.364 & 0.440 & 0.464 \\
    Qwen2.5 & 14B & original & 0.798 & 0.745 & 0.627 & 0.836 & 0.902 & 0.916 & 0.868 & 0.833 & 0.871 & 0.829 & 0.698 & 0.836 & 0.898 & 0.609 & 0.901 & 0.825 & 0.790 & 0.853 & 0.769 & 0.620 & 0.803 & 0.942 & 0.944 & 0.900 & 0.900 & 0.840 & 0.649 & 0.860 & 0.578 & 0.872 & 0.684 & 0.914 & 0.964 & 0.851 & 0.933 & 0.923 & 0.901 & 0.827 & 0.691 & 0.841 & 0.900 & 0.940 & 0.779 & 0.630 & 0.756 & 0.908 & 0.917 & 0.560 & 0.710 & 0.560 & 0.637 & 0.800 & 0.851 & 0.779 & 0.870 & 0.916 & 0.719 & 0.900 & 0.659 & 0.669 & 0.796 & 0.705 \\
    Qwen2.5 & 14B & wickd & 0.709 & 0.661 & 0.659 & 0.770 & 0.887 & 0.886 & 0.661 & 0.769 & 0.712 & 0.665 & 0.603 & 0.736 & 0.796 & 0.554 & 0.708 & 0.737 & 0.670 & 0.762 & 0.671 & 0.540 & 0.695 & 0.767 & 0.761 & 0.810 & 0.824 & 0.752 & 0.585 & 0.849 & 0.518 & 0.784 & 0.614 & 0.778 & 0.912 & 0.749 & 0.853 & 0.875 & 0.756 & 0.732 & 0.618 & 0.722 & 0.826 & 0.820 & 0.682 & 0.620 & 0.644 & 0.789 & 0.819 & 0.550 & 0.600 & 0.540 & 0.578 & 0.660 & 0.723 & 0.641 & 0.725 & 0.842 & 0.675 & 0.820 & 0.519 & 0.616 & 0.699 & 0.607 \\
    Qwen2.5-Instruct & 14B & original & 0.800 & 0.748 & 0.627 & 0.861 & 0.922 & 0.895 & 0.909 & 0.870 & 0.877 & 0.824 & 0.737 & 0.807 & 0.901 & 0.593 & 0.889 & 0.826 & 0.800 & 0.860 & 0.763 & 0.620 & 0.816 & 0.874 & 0.940 & 0.870 & 0.909 & 0.846 & 0.652 & 0.857 & 0.584 & 0.874 & 0.711 & 0.909 & 0.964 & 0.849 & 0.916 & 0.910 & 0.916 & 0.837 & 0.718 & 0.857 & 0.910 & 0.920 & 0.779 & 0.690 & 0.741 & 0.895 & 0.917 & 0.530 & 0.730 & 0.570 & 0.618 & 0.820 & 0.843 & 0.779 & 0.854 & 0.906 & 0.724 & 0.910 & 0.656 & 0.722 & 0.801 & 0.705 \\
    Qwen2.5-Instruct & 14B & wickd & 0.727 & 0.681 & 0.635 & 0.806 & 0.902 & 0.857 & 0.727 & 0.806 & 0.767 & 0.668 & 0.661 & 0.756 & 0.806 & 0.555 & 0.789 & 0.757 & 0.700 & 0.785 & 0.688 & 0.550 & 0.722 & 0.806 & 0.803 & 0.810 & 0.862 & 0.745 & 0.603 & 0.831 & 0.530 & 0.794 & 0.623 & 0.798 & 0.917 & 0.772 & 0.874 & 0.864 & 0.817 & 0.739 & 0.600 & 0.727 & 0.841 & 0.840 & 0.701 & 0.630 & 0.674 & 0.803 & 0.819 & 0.580 & 0.640 & 0.570 & 0.608 & 0.710 & 0.719 & 0.690 & 0.762 & 0.845 & 0.665 & 0.810 & 0.567 & 0.642 & 0.685 & 0.634 \\
    Qwen2.5 & 7B & original & 0.741 & 0.677 & 0.548 & 0.855 & 0.858 & 0.882 & 0.843 & 0.824 & 0.798 & 0.786 & 0.570 & 0.781 & 0.849 & 0.535 & 0.860 & 0.772 & 0.760 & 0.770 & 0.711 & 0.510 & 0.749 & 0.922 & 0.919 & 0.840 & 0.858 & 0.794 & 0.567 & 0.790 & 0.572 & 0.836 & 0.623 & 0.884 & 0.938 & 0.785 & 0.895 & 0.912 & 0.802 & 0.794 & 0.700 & 0.808 & 0.856 & 0.910 & 0.713 & 0.570 & 0.719 & 0.842 & 0.847 & 0.550 & 0.700 & 0.500 & 0.569 & 0.820 & 0.753 & 0.745 & 0.746 & 0.874 & 0.690 & 0.860 & 0.574 & 0.589 & 0.708 & 0.616 \\
    Qwen2.5 & 7B & wickd & 0.484 & 0.454 & 0.508 & 0.612 & 0.745 & 0.709 & 0.455 & 0.546 & 0.448 & 0.436 & 0.364 & 0.434 & 0.432 & 0.408 & 0.497 & 0.499 & 0.480 & 0.408 & 0.457 & 0.450 & 0.484 & 0.427 & 0.457 & 0.490 & 0.517 & 0.556 & 0.443 & 0.757 & 0.343 & 0.529 & 0.465 & 0.530 & 0.565 & 0.479 & 0.525 & 0.618 & 0.481 & 0.539 & 0.409 & 0.494 & 0.502 & 0.520 & 0.468 & 0.420 & 0.452 & 0.546 & 0.514 & 0.430 & 0.350 & 0.360 & 0.471 & 0.490 & 0.506 & 0.448 & 0.487 & 0.516 & 0.488 & 0.600 & 0.407 & 0.371 & 0.505 & 0.384 \\
    Qwen2.5-Instruct & 7B & original & 0.744 & 0.687 & 0.571 & 0.855 & 0.897 & 0.882 & 0.851 & 0.796 & 0.804 & 0.783 & 0.631 & 0.765 & 0.846 & 0.531 & 0.860 & 0.780 & 0.800 & 0.792 & 0.740 & 0.500 & 0.758 & 0.893 & 0.923 & 0.840 & 0.867 & 0.788 & 0.589 & 0.783 & 0.566 & 0.833 & 0.649 & 0.889 & 0.933 & 0.792 & 0.891 & 0.899 & 0.809 & 0.786 & 0.736 & 0.780 & 0.866 & 0.900 & 0.707 & 0.560 & 0.696 & 0.855 & 0.875 & 0.550 & 0.720 & 0.430 & 0.569 & 0.810 & 0.745 & 0.724 & 0.720 & 0.871 & 0.709 & 0.860 & 0.537 & 0.616 & 0.704 & 0.643 \\
    Qwen2.5-Instruct & 7B & wickd & 0.487 & 0.471 & 0.516 & 0.667 & 0.750 & 0.717 & 0.405 & 0.528 & 0.399 & 0.428 & 0.408 & 0.466 & 0.472 & 0.423 & 0.503 & 0.501 & 0.460 & 0.457 & 0.480 & 0.340 & 0.502 & 0.447 & 0.487 & 0.480 & 0.499 & 0.500 & 0.450 & 0.768 & 0.446 & 0.537 & 0.500 & 0.551 & 0.565 & 0.479 & 0.555 & 0.631 & 0.557 & 0.525 & 0.509 & 0.469 & 0.507 & 0.470 & 0.450 & 0.270 & 0.378 & 0.553 & 0.479 & 0.440 & 0.450 & 0.330 & 0.392 & 0.450 & 0.443 & 0.434 & 0.471 & 0.552 & 0.414 & 0.610 & 0.359 & 0.397 & 0.509 & 0.473 \\
    Qwen2.5 & 72B & original & 0.860 & 0.818 & 0.722 & 0.867 & 0.951 & 0.937 & 0.909 & 0.917 & 0.908 & 0.879 & 0.816 & 0.881 & 0.932 & 0.702 & 0.906 & 0.877 & 0.860 & 0.887 & 0.844 & 0.710 & 0.843 & 0.922 & 0.962 & 0.920 & 0.944 & 0.925 & 0.780 & 0.912 & 0.578 & 0.921 & 0.825 & 0.939 & 0.984 & 0.918 & 0.962 & 0.952 & 0.916 & 0.897 & 0.800 & 0.878 & 0.945 & 0.960 & 0.848 & 0.740 & 0.822 & 0.941 & 0.944 & 0.700 & 0.790 & 0.720 & 0.755 & 0.870 & 0.940 & 0.862 & 0.918 & 0.942 & 0.803 & 0.960 & 0.737 & 0.748 & 0.819 & 0.812 \\
    Qwen2.5 & 72B & wickd & 0.789 & 0.749 & 0.683 & 0.855 & 0.941 & 0.920 & 0.736 & 0.852 & 0.822 & 0.743 & 0.704 & 0.788 & 0.864 & 0.672 & 0.743 & 0.811 & 0.730 & 0.819 & 0.786 & 0.520 & 0.753 & 0.825 & 0.786 & 0.890 & 0.913 & 0.843 & 0.720 & 0.908 & 0.566 & 0.851 & 0.711 & 0.869 & 0.927 & 0.851 & 0.933 & 0.927 & 0.824 & 0.812 & 0.691 & 0.751 & 0.871 & 0.870 & 0.768 & 0.660 & 0.741 & 0.862 & 0.924 & 0.640 & 0.730 & 0.670 & 0.735 & 0.750 & 0.843 & 0.745 & 0.775 & 0.894 & 0.778 & 0.890 & 0.622 & 0.669 & 0.755 & 0.732 \\
    gemma-2 & 9B & wickd & 0.572 & 0.433 & 0.460 & 0.600 & 0.745 & 0.705 & 0.446 & 0.556 & 0.454 & 0.425 & 0.279 & 0.408 & 0.389 & 0.419 & 0.456 & 0.497 & 0.480 & 0.400 & 0.486 & 0.400 & 0.525 & 0.476 & 0.466 & 0.520 & 0.511 & 0.536 & 0.397 & 0.754 & 0.349 & 0.533 & 0.482 & 0.551 & 0.575 & 0.479 & 0.529 & 0.618 & 0.504 & 0.538 & 0.473 & 0.461 & 0.507 & 0.540 & 0.446 & 0.300 & 0.496 & 0.513 & 0.549 & 0.430 & 0.290 & 0.340 & 0.441 & 0.460 & 0.511 & 0.441 & 0.389 & 0.545 & 0.458 & 0.510 & 0.367 & 0.338 & 0.537 & 0.402 \\
    gemma-2 & 9B & original & 0.710 & 0.637 & 0.508 & 0.800 & 0.882 & 0.865 & 0.860 & 0.833 & 0.828 & 0.772 & 0.387 & 0.775 & 0.784 & 0.542 & 0.860 & 0.763 & 0.740 & 0.789 & 0.699 & 0.510 & 0.803 & 0.874 & 0.906 & 0.810 & 0.849 & 0.768 & 0.525 & 0.779 & 0.560 & 0.833 & 0.596 & 0.889 & 0.948 & 0.785 & 0.832 & 0.917 & 0.832 & 0.789 & 0.745 & 0.776 & 0.866 & 0.930 & 0.646 & 0.420 & 0.719 & 0.789 & 0.868 & 0.510 & 0.510 & 0.400 & 0.520 & 0.800 & 0.745 & 0.724 & 0.563 & 0.894 & 0.695 & 0.780 & 0.437 & 0.490 & 0.644 & 0.518 \\
    gemma-2-it & 9B & wickd & 0.484 & 0.469 & 0.492 & 0.612 & 0.740 & 0.743 & 0.413 & 0.565 & 0.442 & 0.442 & 0.425 & 0.412 & 0.420 & 0.427 & 0.485 & 0.494 & 0.430 & 0.419 & 0.457 & 0.440 & 0.511 & 0.456 & 0.474 & 0.530 & 0.508 & 0.507 & 0.433 & 0.746 & 0.331 & 0.537 & 0.482 & 0.581 & 0.565 & 0.451 & 0.550 & 0.606 & 0.511 & 0.556 & 0.455 & 0.506 & 0.522 & 0.500 & 0.446 & 0.330 & 0.481 & 0.526 & 0.556 & 0.420 & 0.310 & 0.240 & 0.441 & 0.490 & 0.494 & 0.476 & 0.392 & 0.545 & 0.498 & 0.520 & 0.378 & 0.338 & 0.477 & 0.420 \\
    gemma-2-it & 9B & original & 0.722 & 0.664 & 0.540 & 0.836 & 0.882 & 0.890 & 0.835 & 0.824 & 0.840 & 0.751 & 0.484 & 0.746 & 0.818 & 0.561 & 0.865 & 0.769 & 0.730 & 0.777 & 0.717 & 0.480 & 0.798 & 0.825 & 0.923 & 0.860 & 0.867 & 0.748 & 0.578 & 0.783 & 0.542 & 0.837 & 0.596 & 0.924 & 0.953 & 0.767 & 0.832 & 0.912 & 0.847 & 0.789 & 0.809 & 0.804 & 0.876 & 0.910 & 0.650 & 0.400 & 0.719 & 0.809 & 0.875 & 0.520 & 0.500 & 0.410 & 0.510 & 0.820 & 0.719 & 0.752 & 0.574 & 0.887 & 0.695 & 0.780 & 0.430 & 0.570 & 0.630 & 0.545 \\
    gemma-2-it & 27B & wickd & 0.684 & 0.639 & 0.556 & 0.800 & 0.892 & 0.886 & 0.711 & 0.806 & 0.718 & 0.711 & 0.489 & 0.714 & 0.741 & 0.554 & 0.737 & 0.726 & 0.690 & 0.728 & 0.624 & 0.470 & 0.709 & 0.767 & 0.791 & 0.860 & 0.817 & 0.709 & 0.578 & 0.816 & 0.542 & 0.781 & 0.570 & 0.783 & 0.933 & 0.713 & 0.811 & 0.883 & 0.779 & 0.773 & 0.582 & 0.698 & 0.806 & 0.780 & 0.617 & 0.430 & 0.652 & 0.737 & 0.847 & 0.530 & 0.590 & 0.410 & 0.490 & 0.700 & 0.698 & 0.628 & 0.545 & 0.848 & 0.660 & 0.730 & 0.363 & 0.497 & 0.611 & 0.634 \\
    gemma-2-it & 27B & original & 0.760 & 0.712 & 0.556 & 0.855 & 0.902 & 0.911 & 0.835 & 0.852 & 0.810 & 0.835 & 0.585 & 0.810 & 0.843 & 0.602 & 0.895 & 0.802 & 0.710 & 0.819 & 0.763 & 0.500 & 0.816 & 0.854 & 0.919 & 0.870 & 0.895 & 0.833 & 0.610 & 0.835 & 0.578 & 0.864 & 0.649 & 0.919 & 0.979 & 0.821 & 0.874 & 0.936 & 0.847 & 0.842 & 0.773 & 0.788 & 0.896 & 0.930 & 0.689 & 0.480 & 0.770 & 0.862 & 0.903 & 0.520 & 0.640 & 0.460 & 0.510 & 0.800 & 0.804 & 0.724 & 0.611 & 0.929 & 0.714 & 0.830 & 0.437 & 0.563 & 0.690 & 0.634 \\
    \bottomrule
    \end{tabular}
    \caption{Detailed models performance on the original MMLU sub-tasks }

    \label{tab:sba-vs-sca}
\end{sidewaystable}
    

==> latex/tables/sba_percentages.tex <==
\begin{table*}[t!]
% \small
\begin{adjustbox}{max width=1.0\linewidth}
\begin{tabular}{rrrrrr}
\toprule
\textbf{MMLU}&\textbf{MMLU-Pro}&\textbf{MMLU-Redux}&\textbf{TruthfulQA}&\textbf{Commonsense QA} & \textbf{Arc Challenge}\\
\midrule
20.3\%&16.8\%&14.7\%&3.2\%&3.7\%&5.2\%\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{The Percentage of Single Best Answer (SBA) questions in the benchmarks as determined by our SBA classifier. We do not apply \wicd\space to SBA questions as it can break their coherence.
}
\label{tab:sba-percentages}
\end{table*}

==> latex/tables/sba_percentages_detailed.tex <==
\begin{table*}[th!]
% \small
% \centering
\begin{adjustbox}{max width=1.0\linewidth}
\begin{tabular}{rrrrrrr}
\toprule
&\textbf{MMLU}&\textbf{MMLU-Pro}&\textbf{TQA}&\textbf{CSQA}&\textbf{Recall}&\textbf{Precision}\\
\midrule
Manual&17.3 &12.3 &3.3 &3.8 &--&--\\
GPT-4o-mini&18.2 &13 &4.2 &3.9 &98.5 &97.4\\
SBA Classifier &19.6&14.2&4.5&4 &98.9&95.1\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{The Percentage of Single Best Answer (SBA) questions in 1K questions sampled uniformly from  MMLU, MMLU-Pro, TruthfulQA (TQA), and CommonsenseQA (CSQA) as determined by our manual Annotations, GPT-4o-mini, and our trained SBA classifier. Recall and precision are computed with respect to the manual annotation.
}
\label{tab:detailed-sba-percentages}
\end{table*}


% \begin{table}[th!]
% % \small
% % \centering
% \begin{adjustbox}{max width=1.0\columnwidth}
% \begin{tabular}{rrrrrr}
% \toprule
% &\textbf{\benchmarksmall{MMLU}}&\textbf{\benchmarksmall{MMLU-Pro}}&\textbf{\benchmarksmall{TQA}}&\textbf{\benchmarksmall{CSQA}}&\textbf{\benchmarksmall{Recall}}\\
% \midrule
% Manual&17.3 &12.3 &3.3 &3.8 &--\\
% GPT-4o-mini&18.2 &13 &4.2 &3.9 &98.5 \\
% SBA Classifier (ours)&19.6 &14.2 &4.5 &4 &98.9 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{The Percentage of Single Best Answer (SBA) questions in 1K questions sampled uniformly from  MMLU, MMLU-Pro, TruthfulQA (TQA), and CommonsenseQA (CSQA) as determined by our manual Annotations, GPT-4o-mini, and our trained SBA classifier. Recall is computed with respect to the manual annotation
% }
% \label{tab:detailed-sba-percentages}
% \end{table}
